Multi-Frequency Progressive Refinement for Learned Inverse Scattering

Interpreting scattered acoustic and electromagnetic wave patterns is a computational task that enables remote imaging in a number of important applications, including medical imaging, geophysical exploration, sonar and radar detection, and nondestructive testing of materials. However, accurately and stably recovering an inhomogeneous medium from far-field scattered wave measurements is a computationally difficult problem, due to the nonlinear and non-local nature of the forward scattering process. We design a neural network, called Multi-Frequency Inverse Scattering Network (MFISNet), and a training method to approximate the inverse map from far-field scattered wave measurements at multiple frequencies. We consider three variants of MFISNet, with the strongest performing variant inspired by the recursive linearization method--a commonly used technique for stably inverting scattered wavefield data--that progressively refines the estimate with higher frequency content. MFISNet outperforms past methods in regimes with high-contrast, heterogeneous large objects, and inhomogeneous unknown backgrounds.

==> revised_highlights.tex <==
\begin{highlights}
    \item We introduce a neural network architecture and training method that is inspired by recursive linearization algorithms.
    \item We show that our network achieves lower errors than single-frequency methods and multi-frequency methods in the literature as well as other newly-introduced multi-frequency methods in a high-contrast, noiseless, full-aperture setting.
    \item We demonstrate numerically that our method is robust to moderate measurement noise.
    \item We consider alternative training strategies and find that the proposed progressive training strategy made possible by our architecture is important to its performance.
\end{highlights}
